An elementary proof of Novikov's theorem

Novikov's theorem states that, given a taut (codimension-one) foliation on a closed 3-manifold M, the fundamental group of any leaf injects into the fundamental group of M. We use foliated branched covers to give a simple proof of this result.

==> Bibliography <==
@article {Eynard-Bontemps,
    AUTHOR = {Eynard-Bontemps, H\'{e}l\`ene},
    TITLE = {On the connectedness of the space of codimension one
    foliations on a closed 3-manifold},
    JOURNAL = {Invent. Math.},
    FJOURNAL = {Inventiones Mathematicae},
    VOLUME = {204},
    YEAR = {2016},
    NUMBER = {2},
    PAGES = {605--670},
    ISSN = {0020-9910},
    MRCLASS = {57R30},
    MRNUMBER = {3489706},
    MRREVIEWER = {Pablo Lessa},
    DOI = {10.1007/s00222-015-0622-8},
    URL = {https://doi-org.ezproxy.ulb.ac.be/10.1007/s00222-015-0622-8},
}

@article {Meigniez,
    AUTHOR = {Meigniez, Ga\"{e}l},
    TITLE = {Regularization and minimization of codimension-one {H}aefliger
    structures},
    JOURNAL = {J. Differential Geom.},
    FJOURNAL = {Journal of Differential Geometry},
    VOLUME = {107},
    YEAR = {2017},
    NUMBER = {1},
    PAGES = {157--202},
    ISSN = {0022-040X},
    MRCLASS = {57R30 (57R45)},
    MRNUMBER = {3698236},
    MRREVIEWER = {Robert Roussarie},
    DOI = {10.4310/jdg/1505268031},
    URL = {https://doi-org.ezproxy.ulb.ac.be/10.4310/jdg/1505268031},
}

@article {Hass,
    AUTHOR = {Hass, Joel},
    TITLE = {Minimal surfaces in foliated manifolds},
    JOURNAL = {Comment. Math. Helv.},
    FJOURNAL = {Commentarii Mathematici Helvetici},
    VOLUME = {61},
    YEAR = {1986},
    NUMBER = {1},
    PAGES = {1--32},
    ISSN = {0010-2571},
    MRCLASS = {53A10 (57R30)},
    MRNUMBER = {847517},
    MRREVIEWER = {J. H. Rubinstein},
    DOI = {10.1007/BF02621899},
    URL = {https://doi-org.ezproxy.ulb.ac.be/10.1007/BF02621899},
}

@article {Sullivan1,
    AUTHOR = {Sullivan, Dennis},
    TITLE = {Cycles for the dynamical study of foliated manifolds and
    complex manifolds},
    JOURNAL = {Invent. Math.},
    FJOURNAL = {Inventiones Mathematicae},
    VOLUME = {36},
    YEAR = {1976},
    PAGES = {225--255},
    ISSN = {0020-9910},
    MRCLASS = {57D15},
    MRNUMBER = {433464},
    MRREVIEWER = {Robert Roussarie},
    DOI = {10.1007/BF01390011},
    URL = {https://doi-org.ezproxy.ulb.ac.be/10.1007/BF01390011},
}
    
@article {Sullivan2,
    AUTHOR = {Sullivan, Dennis},
    TITLE = {A homological characterization of foliations consisting of
                  minimal surfaces},
    JOURNAL = {Comment. Math. Helv.},
    FJOURNAL = {Commentarii Mathematici Helvetici},
    VOLUME = {54},
    YEAR = {1979},
    NUMBER = {2},
    PAGES = {218--223},
    ISSN = {0010-2571},
    MRCLASS = {57R30},
    MRNUMBER = {535056},
    MRREVIEWER = {Bruce L. Reinhart},
    DOI = {10.1007/BF02566269},
    URL = {https://doi-org.ezproxy.ulb.ac.be/10.1007/BF02566269},
}    

@book {EliMisch,
    AUTHOR = {Eliashberg, Y. and Mishachev, N.},
     TITLE = {Introduction to the {$h$}-principle},
    SERIES = {Graduate Studies in Mathematics},
    VOLUME = {48},
 PUBLISHER = {American Mathematical Society, Providence, RI},
      YEAR = {2002},
     PAGES = {xviii+206},
      ISBN = {0-8218-3227-1},
   MRCLASS = {53D99 (57R17 58E99)},
  MRNUMBER = {1909245},
MRREVIEWER = {John B. Etnyre},
       DOI = {10.1090/gsm/048},
       URL = {https://doi.org/10.1090/gsm/048},
}

@article {Hirsch59,
    AUTHOR = {Hirsch, Morris W.},
     TITLE = {Immersions of manifolds},
   JOURNAL = {Trans. Amer. Math. Soc.},
  FJOURNAL = {Transactions of the American Mathematical Society},
    VOLUME = {93},
      YEAR = {1959},
     PAGES = {242--276},
      ISSN = {0002-9947},
   MRCLASS = {57.00},
  MRNUMBER = {119214},
MRREVIEWER = {M. A. Kervaire},
       DOI = {10.2307/1993453},
       URL = {https://doi.org/10.2307/1993453},
}

@book {Rudin,
    AUTHOR = {Rudin, Walter},
     TITLE = {Principles of mathematical analysis},
    SERIES = {International Series in Pure and Applied Mathematics},
   EDITION = {Third},
 PUBLISHER = {McGraw-Hill Book Co., New York-Auckland-D\"{u}sseldorf},
      YEAR = {1976},
     PAGES = {x+342},
   MRCLASS = {26-02},
  MRNUMBER = {0385023},
}

@article {Calegari,
    AUTHOR = {Calegari, Danny},
     TITLE = {Taut foliations leafwise branch cover {$S^2$}},
   JOURNAL = {Algebr. Geom. Topol.},
  FJOURNAL = {Algebraic \& Geometric Topology},
    VOLUME = {21},
      YEAR = {2021},
    NUMBER = {5},
     PAGES = {2523--2541},
      ISSN = {1472-2747},
   MRCLASS = {57R30 (57M12)},
  MRNUMBER = {4334518},
       DOI = {10.2140/agt.2021.21.2523},
       URL = {https://doi-org.ezproxy.ulb.ac.be/10.2140/agt.2021.21.2523},
}

@article {Novikov,
    AUTHOR = {Novikov, S. P.},
     TITLE = {The topology of foliations},
   JOURNAL = {Trudy Moskov. Mat. Ob\v{s}\v{c}.},
  FJOURNAL = {Trudy Moskovskogo Matemati\v{c}eskogo Ob\v{s}\v{c}estva},
    VOLUME = {14},
      YEAR = {1965},
     PAGES = {248--278},
      ISSN = {0134-8663},
   MRCLASS = {57.36},
  MRNUMBER = {0200938},
MRREVIEWER = {B. L. Reinhart},
}

@article {IbortTorres,
    AUTHOR = {Ibort, Alberto and Mart\'{\i}nez Torres, David},
     TITLE = {Lefschetz pencil structures for 2-calibrated manifolds},
   JOURNAL = {C. R. Math. Acad. Sci. Paris},
  FJOURNAL = {Comptes Rendus Math\'{e}matique. Acad\'{e}mie des Sciences. Paris},
    VOLUME = {339},
      YEAR = {2004},
    NUMBER = {3},
     PAGES = {215--218},
      ISSN = {1631-073X},
   MRCLASS = {53D35 (57R17)},
  MRNUMBER = {2078077},
MRREVIEWER = {Ivan Smith},
       DOI = {10.1016/j.crma.2004.05.018},
       URL = {https://doi-org.ezproxy.ulb.ac.be/10.1016/j.crma.2004.05.018},
}

@article {Eliashberg_Complexification,
    AUTHOR = {Eliashberg, Ya. M.},
     TITLE = {Complexification of contact structures on {$3$}-dimensional
              manifolds},
   JOURNAL = {Uspekhi Mat. Nauk},
  FJOURNAL = {Akademiya Nauk SSSR i Moskovskoe Matematicheskoe Obshchestvo.
              Uspekhi Matematicheskikh Nauk},
    VOLUME = {40},
      YEAR = {1985},
    NUMBER = {6(246)},
     PAGES = {161--162},
      ISSN = {0042-1316},
   MRCLASS = {53C15 (32F30 57R15)},
  MRNUMBER = {815508},
MRREVIEWER = {Aurel Bejancu},
}

@book {CandelConlon,
    AUTHOR = {Candel, Alberto and Conlon, Lawrence},
     TITLE = {Foliations. {II}},
    SERIES = {Graduate Studies in Mathematics},
    VOLUME = {23},
 PUBLISHER = {American Mathematical Society, Providence, RI},
      YEAR = {2000},
     PAGES = {xiv+402},
      ISBN = {0-8218-0809-5},
   MRCLASS = {57R30 (37C85)},
  MRNUMBER = {1732868},
MRREVIEWER = {P. G. Walczak},
       DOI = {10.1090/gsm/023},
       URL = {https://doi-org.ezproxy.ulb.ac.be/10.1090/gsm/023},
}

@article {Donaldson,
    AUTHOR = {Donaldson, S. K.},
     TITLE = {Lefschetz pencils on symplectic manifolds},
   JOURNAL = {J. Differential Geom.},
  FJOURNAL = {Journal of Differential Geometry},
    VOLUME = {53},
      YEAR = {1999},
    NUMBER = {2},
     PAGES = {205--236},
      ISSN = {0022-040X},
   MRCLASS = {53D35 (57R17)},
  MRNUMBER = {1802722},
MRREVIEWER = {Burak Ozbagci},
       URL = {http://projecteuclid.org.ezproxy.ulb.ac.be/euclid.jdg/1214425535},
}

@incollection {Ghys,
    AUTHOR = {Ghys, \'{E}tienne},
     TITLE = {Laminations par surfaces de {R}iemann},
 BOOKTITLE = {Dynamique et g\'{e}om\'{e}trie complexes ({L}yon, 1997)},
    SERIES = {Panor. Synth\`eses},
    VOLUME = {8},
     PAGES = {ix, xi, 49--95},
 PUBLISHER = {Soc. Math. France, Paris},
      YEAR = {1999},
   MRCLASS = {37F75 (30F10 57M50 57R30)},
  MRNUMBER = {1760843},
MRREVIEWER = {Laurent Meersseman},
}

@book {Milnor,
    AUTHOR = {Milnor, J.},
     TITLE = {Morse theory},
    SERIES = {Annals of Mathematics Studies, No. 51},
      NOTE = {Based on lecture notes by M. Spivak and R. Wells},
 PUBLISHER = {Princeton University Press, Princeton, N.J.},
      YEAR = {1963},
     PAGES = {vi+153},
   MRCLASS = {57.50 (53.72)},
  MRNUMBER = {0163331},
MRREVIEWER = {H. I. Levine},
}

@book {Guillemin-Pollack,
    AUTHOR = {Guillemin, Victor and Pollack, Alan},
     TITLE = {Differential topology},
 PUBLISHER = {Prentice-Hall, Inc., Englewood Cliffs, N.J.},
      YEAR = {1974},
     PAGES = {xvi+222},
   MRCLASS = {58-01 (57-01)},
  MRNUMBER = {0348781},
MRREVIEWER = {K. H. Mayer},
}

@book {Munkres,
    AUTHOR = {Munkres, James R.},
     TITLE = {Topology},
      NOTE = {Second edition of [ MR0464128]},
 PUBLISHER = {Prentice Hall, Inc., Upper Saddle River, NJ},
      YEAR = {2000},
     PAGES = {xvi+537},
      ISBN = {0-13-181629-2},
   MRCLASS = {54-01},
  MRNUMBER = {3728284},
}

@article {Rosenberg,
    AUTHOR = {Rosenberg, Harold},
     TITLE = {Foliations by planes},
   JOURNAL = {Topology},
  FJOURNAL = {Topology. An International Journal of Mathematics},
    VOLUME = {7},
      YEAR = {1968},
     PAGES = {131--138},
      ISSN = {0040-9383},
   MRCLASS = {57.36},
  MRNUMBER = {228011},
MRREVIEWER = {J. W. Smith},
       DOI = {10.1016/0040-9383(68)90021-9},
       URL = {https://doi-org.ezproxy.ulb.ac.be/10.1016/0040-9383(68)90021-9},
}



@book {CalegariBook,
    AUTHOR = {Calegari, Danny},
     TITLE = {Foliations and the geometry of 3-manifolds},
    SERIES = {Oxford Mathematical Monographs},
 PUBLISHER = {Oxford University Press, Oxford},
      YEAR = {2007},
     PAGES = {xiv+363},
      ISBN = {978-0-19-857008-0},
   MRCLASS = {57R30 (37C85 57M50 57N10)},
  MRNUMBER = {2327361},
MRREVIEWER = {Thilo Kuessner},
}


@article {PalaisHomotopy,
    AUTHOR = {Palais, Richard S.},
     TITLE = {Homotopy theory of infinite dimensional manifolds},
   JOURNAL = {Topology},
  FJOURNAL = {Topology. An International Journal of Mathematics},
    VOLUME = {5},
      YEAR = {1966},
     PAGES = {1--16},
      ISSN = {0040-9383},
   MRCLASS = {57.55 (55.40)},
  MRNUMBER = {189028},
MRREVIEWER = {A. Dold},
       DOI = {10.1016/0040-9383(66)90002-4},
       URL = {https://doi-org.ezproxy.ulb.ac.be/10.1016/0040-9383(66)90002-4},
}

@inproceedings {Palais,
    AUTHOR = {Palais, Richard S.},
     TITLE = {Critical point theory and the minimax principle},
 BOOKTITLE = {Global {A}nalysis ({P}roc. {S}ympos. {P}ure {M}ath., {V}ol.
              {XV}, {B}erkeley, {C}alif, 1968)},
     PAGES = {185--212},
 PUBLISHER = {Amer. Math. Soc., Providence, R.I.},
      YEAR = {1970},
   MRCLASS = {57.55 (57.50)},
  MRNUMBER = {0264712},
MRREVIEWER = {D. G. Ebin},
}

@article {Schoen-Yau,
    AUTHOR = {Schoen, Richard and Yau, Shing Tung},
     TITLE = {Existence of incompressible minimal surfaces and the topology of three-dimensional manifolds with nonnegative scalar curvature},
   JOURNAL = {Ann. of Math.},
  FJOURNAL = {Annals of Mathematics},
    VOLUME = {110},
    NUMBER = {1},
      YEAR = {1979},
     PAGES = {127--142},
      ISSN = {0003-486X},
       DOI = {https://doi.org/10.2307/1971247},
       URL = {http://jstor.org/stable/1971247},
}

@article {Meeks-Simon-Yau,
    AUTHOR = {Meeks III, William and Simon, Leon and Yau, Shing Tung},
     TITLE = {Embedded minimal surfaces, exotic spheres, and manifolds with positive Ricci curvature.},
   JOURNAL = {Ann. of Math.},
  FJOURNAL = {Annals of Mathematics},
    VOLUME = {116},
    NUMBER = {3},
      YEAR = {1982},
     PAGES = {621--659},
      ISSN = {0003-486X},
       DOI = {https://doi.org/10.2307/2007026},
       URL = {https://www.jstor.org/stable/2007026},
}


@inbook {Schoen,
    AUTHOR = {Schoen, Richard},
   CHAPTER = {Estimates for stable minimal surfaces in three-dimensional manifolds.},
    SERIES = {Ann. of Math. Stud.},
   FSERIES = {Annals of Mathematics Studies},
     TITLE = {Seminar on minimal submanifolds},
    VOLUME = {103},
    NUMBER = {},
      YEAR = {1983},
 PUBLISHER = {Princeton University Press},
     PAGES = {111--126},
      ISBN = {9780691083247},
      ISSN = {0066-2313},
       DOI = {https://doi.org/10.1515/9781400881437-006},
       URL = {https://www.jstor.org/stable/j.ctt1b7x7tv},
}


@article {Choi-Schoen,
    AUTHOR = {Choi, Hyeong In and Schoen, Richard},
     TITLE = {The space of minimal embeddings of a surface into a three-dimensional manifold of positive Ricci curvature.},
   JOURNAL = {Invent. Math.},
  FJOURNAL = {Inventiones Mathematicae},
    VOLUME = {81},
    NUMBER = {3},
      YEAR = {1985},
     PAGES = {387--349},
      ISSN = {0020-9910},
       DOI = {https://doi.org/10.1007/BF01388577},
       URL = {https://link.springer.com/article/10.1007/BF01388577},
}

@article {Meeks-Yau1,
    AUTHOR = {Meeks III, William and Yau, Shing Tung},
     TITLE = {The classical Plateau problem and the topology of three-dimensional manifolds. The embedding of the solution given by Douglas-Morrey and an analytic proof of Dehn's lemma},
   JOURNAL = {Topology},
  FJOURNAL = {Topology. An International Journal of Mathematics},
    VOLUME = {21},
    NUMBER = {4},
      YEAR = {1982a},
     PAGES = {409--442},
      ISSN = {0129-167X},
       DOI = {https://doi.org/10.2307/1971088},
       URL = {https://www.jstor.org/stable/1971088},
}


@article {Meeks-Yau2,
    AUTHOR = {Meeks III, William and Yau, Shing Tung},
     TITLE = {The existence of embedded minimal surfaces and the problem of uniqueness.},
   JOURNAL = {Math. Z.},
  FJOURNAL = {Mathematische Zeitschrift},
    VOLUME = {179},
    NUMBER = {2},
      YEAR = {1982b},
     PAGES = {151--168},
      ISSN = {0025-5874},
       DOI = {https://doi.org/10.1007/BF01214308},
       URL = {https://link.springer.com/article/10.1007/BF01214308},
}


@article {Hass-Scott,
    AUTHOR = {Hass, Joal and Scott, Peter},
     TITLE = {The existence of least area surfaces in 3-manifolds.},
   JOURNAL = {Trans. Amer. Math. Soc.},
  FJOURNAL = {Transactions of the American Mathematical Society},
    VOLUME = {310},
    NUMBER = {1},
      YEAR = {1988},
     PAGES = {87--114},
      ISSN = {0002-9947},
       DOI = {https://doi.org/10.1090/S0002-9947-1988-0965747-6},
       URL = {https://www.ams.org/journals/tran/1988-310-01/S0002-9947-1988-0965747-6},
}

@article {Thurston,
    AUTHOR = {Thurston, W. P.},
     TITLE = {Existence of codimension-one foliations},
   JOURNAL = {Ann. of Math. (2)},
  FJOURNAL = {Annals of Mathematics. Second Series},
    VOLUME = {104},
      YEAR = {1976},
    NUMBER = {2},
     PAGES = {249--268},
      ISSN = {0003-486X},
   MRCLASS = {57D30},
  MRNUMBER = {425985},
MRREVIEWER = {D. B. Fuchs},
       DOI = {10.2307/1971047},
       URL = {https://doi-org.ezproxy.ulb.ac.be/10.2307/1971047},
}



@book {Moerdijk,place={Cambridge}, series={Cambridge Studies in Advanced Mathematics}, title={Introduction to Foliations and Lie Groupoids}, DOI={10.1017/CBO9780511615450}, publisher={Cambridge University Press}, author={Moerdijk, I. and Mrcun, J.}, year={2003}, collection={Cambridge Studies in Advanced Mathematics}}

@book{Geiges, place={Cambridge}, series={Cambridge Studies in Advanced Mathematics}, title={An Introduction to Contact Topology}, DOI={10.1017/CBO9780511611438}, publisher={Cambridge University Press}, author={Geiges, Hansjörg}, year={2008}, collection={Cambridge Studies in Advanced Mathematics}}

@book {EliashbergThurston, title = {Confoliations}, author = {Eliashberg, Yakov and Thurston, William P.}, publisher = {American Mathematical Society}, year = {1998}}

@misc {CalcPlot3D,
  author = {Seeburger, Paul},
    title = {CalcPlot3D},
  year = 2018,
  howpublished = {https://c3d.libretexts.org/CalcPlot3D/index.html},
  note = {Project website: https://sites.monroecc.edu/multivariablecalculus/},
  urldate = {2022-04-23}

}

@article{Rummler1979,
author = {Rummler, Hansklaus},
journal = {Commentarii mathematici Helvetici},
keywords = {Foliation By Minimal Submanifolds; Hausdorff Foliation; F-Closed Forms},
pages = {224-239},
title = {Quelques notions simples en g\'eom\'etrie riemannienne et leurs applications aux feuilletages compacts.},
url = {http://eudml.org/doc/139781},
volume = {54},
year = {1979},
}


@article{Haefliger,
     author = {Haefliger, Andr\'e},
     title = {Vari\'et\'es feuillet\'ees},
     journal = {Annali della Scuola Normale Superiore di Pisa - Classe di Scienze},
     pages = {367--397},
     publisher = {Scuola normale superiore},
     volume = {3e s{\'e}rie, 16},
     number = {4},
     year = {1962},
     zbl = {0122.40702},
     mrnumber = {189060},
     language = {fr},
     url = {http://www.numdam.org/item/ASNSP_1962_3_16_4_367_0/}
}

@book{doCarmo,
  title={Riemannian Geometry},
  author={do Carmo, M.P.},
  isbn={9783764334901},
  lccn={91037377},
  series={Mathematics (Boston, Mass.)},
  url={https://books.google.es/books?id=uXJQQgAACAAJ},
  year={1992},
  publisher={Birkh{\"a}user}
}


@article{Riemann,
  abstract = {Plan of the Investigation.
It is known that geometry assumes, as things given, both the notion of space and the first principles of constructions in space. She gives definitions of them which are merely nominal, while the true determinations appear in the form of axioms. The relation of these assumptions remains consequently in darkness; we neither perceive whether and how far their connection is necessary, nor a priori, whether it is possible. },
  added-at = {2012-04-21T00:52:04.000+0200},
  address = {London},
  author = {Riemann, Bernhard},
  biburl = {https://www.bibsonomy.org/bibtex/2594b40ddeb8177738ce5a0329f291e1e/cenderjk},
  description = {Original and translation of Bernhard Riemann's Habilitation lecture of 1854, Ueber die Hypothesen, welche der Geometrie zu Grunde liegen, published by Richard Dedekind after Riemann's death, in Abhandlungen der Königlichen Gesellschaft der Wissenschaften zu Göttingen, vol. 13, 1867.},
  editor = {{Clifford, William Kingdon}, trans.},
  interhash = {1c2d669870c72609f8cc09e63664e943},
  intrahash = {594b40ddeb8177738ce5a0329f291e1e},
  journal = {Nature},
  keywords = {Riemann geometry hypotheses},
  month = may,
  note = {doi:10.1038/008014a0},
  number = {183, 184},
  pages = {14-17, 36, 37},
  refid = {doi:10.1038/008014a0},
  timestamp = {2012-04-21T00:59:09.000+0200},
  title = {On the hypotheses which lie at the bases of geometry},
  url = {http://www.maths.tcd.ie/pub/HistMath/People/Riemann/Geom/},
  volume = {VIII},
  year = 1873
}



@Book{Hirsch,
author = { Hirsch, Morris W.},
title = { Differential topology },
edition = { Corr. 6th print. },
isbn = { 0387901485 3540901485 },
publisher = { Springer New York },
pages = { x, 222 p. : },
year = { 1997 },
type = { Book },
language = { English },
subjects = { Differential topology. },
life-dates = { 1997 -  },
catalogue-url = { https://nla.gov.au/nla.cat-vn617993 },
}


 @inbook{SteinShakarchi, place={Princeton}, series={Princeton lectures in analysis }, chapter={Weyl's equidistribution theorem}, volume={I}, title={Fourier analysis}, publisher={Princeton university press}, author={Stein, M. and Shakarchi, Rami}, year={2003}, pages={105–113}, collection={Princeton lectures in analysis }} 
 
  @book{CamachoNeto, place={Boston, Massachusetts}, title={Geometric theory of foliations}, publisher={Birkh\"auser}, author={Camacho, C\'esar and Neto, Lins Alcides}, year={1985}} 
  
  @phdthesis{ReebThesis,
  author       = {Reeb, Georges}, 
  title        = {Sur certaines propri\'et\'es topologiques des vari\'et\'es feuillet\'ees},
  school       = {Universit\'e de Strasbourg},
  year         = {1952},
  address      = {Hermann et Cie, \'editeurs, 6, rue de la Sorbonne, Paris},
}

@Article{Ehresmann-Shih,
 Author = {Ehresmann, Charles and Shih, Weishu},
 Title = {Sur les espaces feuillet{\'e}s: th{\'e}or{\`e}me de stabilit{\'e}},
 FJournal = {Comptes Rendus Hebdomadaires des S{\'e}ances de l'Acad{\'e}mie des Sciences, Paris},
 Journal = {C. R. Acad. Sci., Paris},
 ISSN = {0001-4036},
 Volume = {243},
 Pages = {344--346},
 Year = {1956},
 Language = {French},
 zbMATH = {3118066},
 Zbl = {0070.40102}
}

 @article{haefliger1958, title={Structures Feuilletées et cohomologie à valeur dans un faisceau de groupoïdes}, volume={32}, DOI={10.1007/bf02564582}, number={1}, journal={Commentarii Mathematici Helvetici}, author={Haefliger, André}, year={1958}, pages={248–329}} 
 
 @article{EpsteinMillettTischler,
author = {Epstein, D. and Millett, Kenneth and Tischler, D.},
year = {1977},
month = {12},
pages = {548-552},
title = {Leaves Without Holonomy},
volume = {16},
journal = {Journal of The London Mathematical Society-second Series - J LONDON MATH SOC-SECOND SER},
doi = {10.1112/jlms/s2-16.3.548}
}

 @article{goodman1975, title={Closed leaves in foliations of codimension one}, volume={50}, DOI={10.1007/bf02565757}, number={1}, journal={Commentarii Mathematici Helvetici}, author={Goodman, Sue E.}, year={1975}, pages={383–388}} 
